Double-Dipping: A New Relation between Stellar Rotation and Starspot Activity

We report the discovery of a new relationship between a simple morphological characteristic of light curves produced by starspots and stellar rotation periods. The characteristic we examine is whether the light curve exhibits one dip or two during a single rotation. We analyze thousands of Kepler light curves of main sequence stars from 3200-6200K. Almost all the stars exhibit segments of their light curve that contain either single or double dip segments (very few have more than two significant dips per rotation). We define a variable, the "single/double ratio" (SDR) that expresses the ratio of the time spent in single mode to the time spent in double mode. Unexpectedly, there is a strong relationship between the SDR and the stellar rotation period, in the sense that longer periods come with a larger fraction of double segments. Even more unexpectedly, the slopes of the SDR-Period relations are a clear function of stellar temperature. We also show that the relationships of spot variability amplitude (R_var) to rotation period have similar levels of scatter, slopes, and dependence on temperature as the SDR-Period relations. Finally, the median R_var of single segments tends to be about twice that of double segments in a given light curve. We offer some tentative interpretations of these new results in terms of starspot coverage and lifetimes. It will be fruitful to look further into this novel "rotation-activity" relation, and better understand what information these aspects of light curve morphology bring to our knowledge of stellar magnetic activity.

==> table.tex <==
%%
%% Begining of file `table.tex'

%% This complex but short example prepared in the deluxetable environment
%% demonstrates some of the techniques
%% that can be used to generate complex column headings and to align
%% variable-width columns. See the manuscript sample file, sample.tex,
%% for more table examples.

%% Note this file has its own \documentclass, \begin{document}, and
%% \end{document} commands. If you want to insert this table in another
%% LaTeX document using the \input command, comment out these lines.

%\documentclass{aastex}
%\begin{document}

%% Note that the table will print double-spaced since we are using the
%% manuscript style. Change the style to preprint or preprint2 to see
%% how LaTeX formats the table in those styles.

%% In this example the LaTeX \multicolumn command is used to span a heading
%% over several columns.  When \multicolumn is used along with the
%% \cutinhead or \sidehead commands, the \tablecolumns command must
%% be used to specify the number of columns in the table -
%% otherwise \cutinhead and \sidehead will not work properly.

%% \cline has been used to produce straddle rules below the spanning heads,
%% \cutinhead to produce a centered head in the body of the table, and
%% \sidehead to produce a flush-left head in the body.

%% This table also makes use of the \phn command to better align some of the
%% columns.  Also see \phd, \phs, and \phm{} - other commands useful for
%% column alignment.  All of these commands insert a blank space
%% whose width is  equal to that of a number (\phn),
%% a decimal point (\phd), a minus sign (\phs), or any
%% character you wish to use (\phm{text}).
%% Keep in mind that if you are preparing a table for electronic submission
%% to one of the journals, you need not worry too much about column
%% alignment. The editors will fix table alignment as appropriate.

%% If a table is more than one page long, the width of the table can vary
%% from page to page when the default \tablewidth is used, as below.  The
%% individual table widths for each page will be written to the log file; a
%% maximum tablewidth for the table can be computed from these values.
%% The \tablewidth argument can then be reset and the file reprocessed, so
%% that the table is uniform throughout the pages. Try getting the widths
%% from the log file and changing the \tablewidth parameter to see how
%% adjusting this value affects table formatting.

%% The * option to the \\ command has been used in the lines after
%% the \sidehead to keep them together on the same page. Try taking
%% the *'s out and LaTeXing the manuscript again to see the difference
%% in the page breaks. You can group together as many lines as
%% you like using this command.

\begin{deluxetable}{rrrrrrrr}
\tablecolumns{8}
\tablewidth{0pc}
\tablecaption{Percentage of Fake Stars Lost}
\tablehead{
\colhead{}    &  \multicolumn{3}{c}{Non-shell Stars} &   \colhead{}   &
\multicolumn{3}{c}{Shell Stars} \\
\cline{2-4} \cline{6-8} \\
\colhead{Mag} & \colhead{F336W}   & \colhead{F555W}    & \colhead{F814W} &
\colhead{}    & \colhead{F336W}   & \colhead{F555W}    & \colhead{F814W}}
\startdata
20.25 & 2.2$\pm$7.4\phn & \nodata & \nodata &
& 0.9$\pm$6.8 & \nodata & 0.0$\pm$44.7 \\
20.75 & 2.4$\pm$7.8\phn & \nodata & 2.8$\pm$7.4 &
& 1.7$\pm$6.6 & \nodata & 1.4$\pm$6.7\phn \\
21.25 & 0.1$\pm$7.7\phn & \nodata & 1.7$\pm$7.6 &
& 2.6$\pm$6.5 & \nodata & 0.9$\pm$6.6\phn \\
21.75 & 2.4$\pm$4.5\phn & 2.2$\pm$7.4 & 0.1$\pm$7.6 &
& 7.1$\pm$4.5 & 0.9$\pm$6.8 & 3.3$\pm$6.5\phn \\
22.25 & 3.4$\pm$3.1\phn & 1.8$\pm$7.7 & 2.9$\pm$4.4 &
& 11.8$\pm$3.6 & 0.4$\pm$6.6 & 5.7$\pm$4.4\phn \\
22.75 & 4.5$\pm$2.9\phn & 1.8$\pm$7.7 & 4.7$\pm$3.1 &
& 26.2$\pm$3.6 & 3.4$\pm$6.5 & 10.9$\pm$3.6\phn \\
23.25 & 7.0$\pm$2.4\phn & 3.4$\pm$4.5 & 3.7$\pm$2.9 &
& 44.2$\pm$3.3 & 10.7$\pm$4.5 & 20.6$\pm$3.5\phn \\
\cutinhead{More Data}
23.75 & 12.4$\pm$2.7\phn & 4.1$\pm$3.1 & 6.7$\pm$2.5 &
& 59.8$\pm$4.0 & 20.1$\pm$3.6 & 32.6$\pm$3.4\phn \\
24.25 & 30.2$\pm$3.1\phn & 5.3$\pm$2.9 & 10.0$\pm$2.7 &
& 74.9$\pm$5.1 & 35.8$\pm$3.6 & 43.1$\pm$4.0\phn \\
24.75 & 66.8$\pm$5.5\phn & 10.4$\pm$2.4 & 16.5$\pm$3.2 &
& 83.7$\pm$6.1 & 56.3$\pm$3.3 & 57.0$\pm$5.2\phn \\
25.25 & 87.5$\pm$35.4 & 20.0$\pm$2.7 & 28.0$\pm$5.6 &
& \nodata & 71.5$\pm$4.0 & 71.8$\pm$6.2\phn \\
25.75 & \nodata\phn & 55.3$\pm$3.1 & \nodata &
& \nodata & 81.2$\pm$5.1 & \nodata\phn \\
26.25 & \nodata\phn & 85.1$\pm$5.5 & \nodata &
& \nodata & 85.6$\pm$6.1 & \nodata\phn \\
\sidehead{More Data}
27.75 & 12.4$\pm$2.7\phn & 4.1$\pm$3.1 & 6.7$\pm$2.5 &
& 59.8$\pm$4.0 & 20.1$\pm$3.6 & 32.6$\pm$3.4\phn \\*
28.25 & 30.2$\pm$3.1\phn & 5.3$\pm$2.9 & 10.0$\pm$2.7 &
& 74.9$\pm$5.1 & 35.8$\pm$3.6 & 43.1$\pm$4.0\phn \\*
29.75 & 66.8$\pm$5.5\phn & 10.4$\pm$2.4 & 16.5$\pm$3.2 &
& 83.7$\pm$6.1 & 56.3$\pm$3.3 & 57.0$\pm$5.2\phn \\
30.25 & 87.5$\pm$35.4 & 20.0$\pm$2.7 & 28.0$\pm$5.6 &
& \nodata & 71.5$\pm$4.0 & 71.8$\pm$6.2\phn \\
31.75 & \nodata\phn & 55.3$\pm$3.1 & \nodata &
& \nodata & 81.2$\pm$5.1 & \nodata\phn \\
32.25 & \nodata\phn & 85.1$\pm$5.5 & \nodata &
& \nodata & 85.6$\pm$6.1 & \nodata\phn \\
33.75 & 12.4$\pm$2.7\phn & 4.1$\pm$3.1 & 6.7$\pm$2.5 &
& 59.8$\pm$4.0 & 20.1$\pm$3.6 & 32.6$\pm$3.4\phn \\
34.25 & 30.2$\pm$3.1\phn & 5.3$\pm$2.9 & 10.0$\pm$2.7 &
& 74.9$\pm$5.1 & 35.8$\pm$3.6 & 43.1$\pm$4.0\phn \\
35.75 & 66.8$\pm$5.5\phn & 10.4$\pm$2.4 & 16.5$\pm$3.2 &
& 83.7$\pm$6.1 & 56.3$\pm$3.3 & 57.0$\pm$5.2\phn \\
36.25 & 87.5$\pm$35.4 & 20.0$\pm$2.7 & 28.0$\pm$5.6 &
& \nodata & 71.5$\pm$4.0 & 71.8$\pm$6.2\phn \\
37.75 & \nodata\phn & 55.3$\pm$3.1 & \nodata &
& \nodata & 81.2$\pm$5.1 & \nodata\phn \\
38.25 & \nodata\phn & 85.1$\pm$5.5 & \nodata &
& \nodata & 85.6$\pm$6.1 & \nodata\phn \\
\enddata
\end{deluxetable}

% \end{document}

%%
%% End of file `table.tex'.

